Ascend-CC: Confidential Computing on Heterogeneous NPU for Emerging Generative AI Workloads

Cloud workloads have dominated generative AI based on large language models (LLM). Specialized hardware accelerators, such as GPUs, NPUs, and TPUs, play a key role in AI adoption due to their superior performance over general-purpose CPUs. The AI models and the data are often highly sensitive and come from mutually distrusting parties. Existing CPU-based TEEs such as Intel SGX or AMD SEV do not provide sufficient protection. Device-centric TEEs like Nvidia-CC only address tightly coupled CPU-GPU systems with a proprietary solution requiring TEE on the host CPU side. On the other hand, existing academic proposals are tailored toward specific CPU-TEE platforms. To address this gap, we propose Ascend-CC, a confidential computing architecture based on discrete NPU devices that requires no trust in the host system. Ascend-CC provides strong security by ensuring data and model encryption that protects not only the data but also the model parameters and operator binaries. Ascend-CC uses delegation-based memory semantics to ensure isolation from the host software stack, and task attestation provides strong model integrity guarantees. Our Ascend-CC implementation and evaluation with state-of-the-art LLMs such as Llama2 and Llama3 shows that Ascend-CC introduces minimal overhead with no changes in the AI software stack.

==> sections/ascendCC.tex <==
\section{\ascendcc: End-to-end System}
\label{sec:ascendcc}

\begin{figure*}[t]
    \centering
    \begin{minipage}{.7\textwidth}
        \centering
        \includegraphics[trim=0cm 12.2cm 7.6cm 0cm, clip,width=1\linewidth]{figures/system-design_V2.pdf}
        % \caption{Overall system design}
        % \label{fig:systemdesign}
    \end{minipage}%
    \begin{minipage}{.4\textwidth}
        % \centering
        \includegraphics[trim=-2cm 9.4cm 23cm 0cm, clip,width=0.8\linewidth]{figures/tensor_execute.pdf}
        % \caption{\ascendcc{} PyTorch interface}
        % \label{fig:programming_interface}
    \end{minipage}%    
    \caption{\ascendcc{} end-to-end system design with all internal confidential computing mechanisms along with the corresponding python interface.}
    \label{fig:systemdesign}
\end{figure*}


% \subsection{Overall System Design}
% \label{sec:overall_system_design}

Typically, the host interacts with the NPU through an NPU driver and runtime bundle that uses DMA and MMIO to transfer data and control.
As we assume that the cloud service provider (CSP) is untrusted, all CSP-provided host systems, including their software stack, such as the OS, hypervisor, NPU driver, and runtime, are also attacker-controlled.
We only assume that the NPU is trusted and the NPU provides hardware root-of-trust (RoT).
\Cref{fig:systemdesign} sketches the overall architecture design of \ascendcc{}, showing the interaction between the model provider, the data provider, and the different components of the NPU, along with the executed code. The example code shows our additional instructions (in red) to ensure confidential training and inference on the encrypted model and data.

\myparagraph{Initial setup} The model provider and the data provider can execute an authenticated Diffie-Hellman key exchange (DHKE) with the NPU over the untrusted host. We designate the keys obtained by the DHKE as $\mathcal{K}_M$ (between NPU and model provider) and $\mathcal{K}_D$ (between NPU and data owner). The NPU stores these two keys on the HSM on-chip.

\myparagraph{Data Preparation} \ascendcc{} requires the data provider to prepare encrypted data with the shared secret $\mathcal{K}_D$ 

% \myparagraph{Example scenario}
% A typical program to load the model and data into the NPU and instruct the NPU to execute that model is as follows.
%  The \texttt{modelFile} is a compiled model file that contains information such as the layers, model parameters, and the operator binaries used by the layers. In the above example scenario, the host uses the NPU driver and runtime to communicate with the NPU. First, the host calls \texttt{loadModel} to send the model file to the NPU. Next, the \texttt{memcpy} API sends the training/inference data used by the model to the NPU. The third argument to \texttt{memcpy} call: \texttt{h2d} or host to device indicates the direction of the DMA operation. After the model and the data are sent to the device, the host calls \texttt{execute} API that indicates the NPU to read the tasks from the task queue one by one and execute them. After the execution is completed, the output of the model operation is written to \texttt{result}, which is then copied back from the NPU to the host.


\begin{enumerate}
    \item[\one] The model provider encrypts the model ($M$) with $\mathcal{K}_M$:  $\mathbb{M} = Enc_{\mathcal{K}_M}(M)$ and sends $\mathbb{M}$ to the untrusted CSP. 
    The encrypted model consists of three parts: plaintext layer information, encrypted parameters, and encrypted operator binaries. The CPS calls the \texttt{loadModel} API to load $\mathbb{M}$ to the NPU's HBM. 
    At the same time, the NPU driver and runtime create tasks from the layer information. Note that the layer information 
    \textit{only} contains the (masked) name of the task. These tasks contain the relevant information for the NPU to execute the operators (\texttt{PC\_START}, compute unit (AI CPU or AI Core), \dots). 
    Identically to the vanilla \texttt{loadModel()} API call, these tasks are written to the NPU's task queue.
    
    \item[\two] Next, the host calls \texttt{attestModel($\mathbb{M}$)}, which is a new API call that we introduce in our proposal. 
    The \texttt{attestModel()} API commands the task scheduler to produce an attestation report of the model on the HBM and tasks on the task queue. 
    The detailed attestation protocol is described in~\Cref{sec:buildingBlocks:integrity}.
    
    \item[\three] After the model attestation is successful, the task scheduler programs the internal SMMU to unmap all the tasks and model memory from the host. 
    Therefore, the host cannot read and write from and to the NPU memory. 
    This is carried out by our new \texttt{lockModel($\mathbb{M}$)} API call, which is part of the \ascendcc{} software TCB.  
    
    \item[\four]  After the model has been attested and the associated memory is locked, the data provider encrypts the data ($D$) with $\mathcal{K}_D$:  $\mathbb{D} = Enc_{\mathcal{K}_D}(D)$ and sends $\mathbb{D}$ to the untrusted CSP.
    
    \item[\five] Similar to step \three, the task scheduler reprograms the SMMU to lock the memory region where the encrypted data $\mathbb{D}$ is located so that the host cannot modify the data anymore. Memory locking also ensures that the host cannot access the data once the data is decrypted in-place by the AI CPU AES-GCM operator.
    
    \item[\six] At this point, the NPU starts decrypt encrypted model $\mathbb{M}$ and data $\mathbb{D}$ on the AI CPU, to respectively derive $M$ and $D$. 
    The decryption operation is in-place with their respective keys $\mathcal{K}_M$ and $\mathcal{K}_D$; therefore, the plaintext model and data overwrite their encrypted counterparts. 
    Note that since the memory is locked (steps 
    \three and \five), the host cannot access $M$ and $D$. The output of the model is $R$ is encrypted: $\mathbb{R} = Enc_{\mathcal{K}_D}(R)$. 
    Note that by default, the memory region where the result $R$ resides is unmapped (by SMMU) from the host. After $\mathbb{R}$ is computed, the task scheduler remaps the region of $\mathbb{R}$ back to the host.
    
    \item[\seven] The host executes \texttt{memcpy} to copy over the encrypted result $\mathbb{R}$ from the NPU to the host.
    
    \item[\eight] If there is no more inference rounds, the AI Core and AI CPU calls \texttt{clean()} API that flashes the internal state of the AI Cores and AI CPUs and zeros out the memory spaces of $M$ and $D$.
    
    \item[\nine] Once the memory is cleared, the task scheduler unlocks the memory so that the host can read and write from/to the NPU memory.
\end{enumerate}




% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=0cm 9.6cm 23cm 0cm, clip,width=0.55\linewidth]{figures/tensor_execute.pdf}
%     \caption{\ascendcc{} PyTorch programming interface}
%     \label{fig:programming_interface}
% \end{figure}


\subsection{Programming Interface}
\label{sec:ascendcc:programming_interface}

Note that all of the changes inside the NPU firmware and driver are completely transparent to higher-level programming, such as the AI software stack PyTorch.
Therefore, from the developer's perspective, there are almost no changes to the existing inference (and even training) workflow. 
\ascendcc{} simply acts as a drop-in-replacement for the AI developers.
There are minimal changes within the PyTorch adapter for Ascend NPU (i.e., \texttt{torch\_npu}) to support the collection of the model attestation. 
\Cref{fig:programming_interface} shows the matrix multiplication example (from~\Cref{fig:mm_example_code}) with all the \ascendcc{} hardening.
Note that the cryptographic operators, memory invariant enforcement, and model and task attestations are completely transparent and, therefore, do not require changes from the developer's side.


\begin{figure}[t]
    \centering
    \includegraphics[trim=0cm 11.3cm 22.5cm 0cm, clip,width=0.7\linewidth]{figures/state-machine.pdf}
    \caption{\ascendcc{} memory lifecycle}
    \label{fig:lifecycle}
\end{figure}


\subsection{\ascendcc{} Lifecycle}
\label{sec:ascendcc:lefecycle}

In summary, the memory lifecycle of \ascendcc{} is depicted in~\Cref{fig:lifecycle} that provides the memory states over subsequent rounds of inference passes.
Typically, the model is loaded once, and then many inference passes (such as a conversation with an LLM chatbot) are run afterward.
Therefore, the memory region associated with the model (parameters, binary, and model operator workspace) needs to be locked and decrypted once and stays locked for the rest of the runtime till the model is unloaded, or an interrupt is encountered.
The data, on the other hand, arrives in a streaming fashion.
The data region is locked, decrypted, and fed to the model execution.
Once the output is generated, it is encrypted with the data owner's key, and the corresponding memory region is unlocked for device-to-host DMA transfer.
At the same time, the input regions are reset (by overwriting them to zero by a dedicated AI CPU operator), and the corresponding memory regions are unlocked. 
After that, the host can transfer the next batch of encrypted input data to the NPU.

\subsection{Emerging Application Scenario: Pay-Per-Inference}
\label{sec:ascendccpay_per_inference}

% \begin{figure}[tpb]
% \centering
% \footnotesize
% \resizebox{0.5\textwidth}{!} {%
%  \input{sections/tikz/pay_per_inference_single}}
% \caption{Secure pay-per-inference}
% \label{fig:pay_per_inference}
% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[trim=0cm 5cm 0cm 0cm, clip,width=0.65\linewidth]{figures/PPI.pdf}
    \caption{Pay-per-inference (PPI) protocol where the data owner can register the input tokens without revealing the input data to the model provider to receive an authentication token.}
    \label{fig:pay_per_inference}
\end{figure*}



Based on our confidential computing mechanism on Ascend NPU, we envision data center-oriented emerging AI applications leveraging the \ascendcc{} capabilities. 
Typically, in the AI-as-a-service scenario, such an inference, a customer pays based on the computing time consumption. This could be either the actual time or the number of tokens (in the query) directly related to the computing time.
We designed a new inference service that we call pay-per-inference (PPI). 
We have the identical attacker model in PPI as the rest of the paper, i.e., we assume that the model, data, and cloud provider are mutually distrusting, and we assume that everything except the specific NPU is trusted.
PPI is an interactive protocol where the data provider can register their inference query tokens (e.g., the question to a chatbot) to the model provider without revealing the actual query.
In return, the data provider acquires a query-related authentication token that is then passed to \ascendcc.
Note that the authentication token is a one-way binding between the specific model and the query token.
The NPU checks the validity of the authentication token along with the actual query. 
If the verification is successful, the NPU will execute the model.

% \subsubsection{Outline of the Mechanism}

% \begin{itemize}[leftmargin=*]
% \item The model owner only sends an encrypted model, and it's only decrypted on the device. Therefore, the model is never leaked to the data provider.
% \item	The data owner only sends the message authentication code or MAC of the data to the model owner. The MAC is a one-way commitment of the data. From the MAC, it is impossible to calculate the data. However, it is also impossible for the data owner to find a collision, i.e., to come up with another data that has the same MAC. Therefore, the data owner does not reveal the data to the model owner, and the data owner cannot cheat.
% \item	The hash of the confidential model ensures that the device has loaded the correct model.
% \item	There could be multiple data and model providers running on the same AI accelerator at the same time while having isolation between them.
% \end{itemize}

The detailed pay-per-inference protocol is depicted in~\Cref{fig:pay_per_inference} involving the model provider, the data owner, and the NPU.


% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=0cm 5cm 13.7cm 0cm, clip,width=\linewidth]{figures/secure_dma.pdf}
%     \caption{\textcolor{red}{not needed anymore}}
%     \label{fig:dma_mmio}
% \end{figure}






% \subsection{Secure DMA and MMIO}
% \label{secLdma_mmio}

% The host communicates with the NPU over DMA and MMIO and can read data or send malicious commands to be executed on the NPU. Therefore, it is crucial to protect the communication interfaces between the host and the NPU. First, we ensure that the host can never start a data transfer either end: both from the host to the NPU or from the NPU to the host, known as the DMA direction. The host can request to send or receive data to the NPU by providing the memory address, length, and direction, rather than directly reading or writing the data. After receiving such a request, the NPU can decide whether to respond to such requests or not. This is achieved in the following steps, as depicted in~\Cref{fig:dma_mmio}.

% \begin{itemize}
% \item[\one] First, we remove all DMA memory mappings from the BAR (base address register) mapping space. These mappings are kept in the DMA registers, as shown in~\Cref{fig:dma_mmio}. This was because the NPU memory is not mapped to the host, and such a mechanism prevents the host from reading or writing directly from and to the NPU memory.

% \item[\two] Typically, all DMA transactions between the host and the NPU are invoked by the \texttt{devdrv\_dma\_copy()} API call that is part of the NPU PCIE driver stack. This API uses host memory to store the DMA submission queue (SQ) and completion queue (CQ). The SQ and SQ contain the DMA commands that are to be executed and the commands that complete execution respectively. Typically, SQ and CQ are on the host-memory side, as the host is the BUS master, and the DMA controller on the host side is responsible for the DMA transaction. However, we want to prevent this from happening so that the host is removed from being the bus master.

% \item[\three] We replace the \texttt{devdrv\_dma\_copy()} API call with \texttt{devdrv\_common\_msg\_send()} API call which is a generic interface to send arbitrary messages between a host and a device. 
% \item[\four] Next, the host side TEE (a confidential VM) and the NPU control CPU execute an authenticated Diffie Hellman key exchange to establish a shared secret. The NPU maintains this shared secret on its dedicated crypto chip.
% \item[\five] Through \texttt{devdrv\_common\_msg\_send()}, the host notifies the NPU about the data (start address and the size), and DMA direction (host to device or device to host), so that the NPU can prepare its own  DMA controller. All the parameters in \texttt{devdrv\_common\_msg\_send()} are encrypted and authenticated using AES-GCM with the shared secret between the host and the NPU. The control CPU on the NPU maintains the SQ and CQ on the NPU memory using the parameters sent from the \texttt{devdrv\_common\_msg\_send()} call after verification of the parameters is successful.
% \item[\six] Based on the DMA direction, the DMA driver on the NPU copies data from the host to the NPU memory or vice versa. After the copy is done, the DMA driver notifies the control CPU. As all the parameters of \texttt{devdrv\_common\_msg\_send()} are authenticated encrypted, a malicious OS or hypervisor cannot send any arbitrary DMA command to the NPU. Note that both the host-side TEE and the NPU control CPU maintain a monotonic counter (starting from an initial random nonce) throughout the communication, therefore, eliminating any chance of replay attacker. 
% \end{itemize}





% \begin{figure}[t]
%     \centering
%     \includegraphics[trim=0cm 10.1cm 24cm 0cm, clip,width=0.6\linewidth]{figures/model_verify.pdf}
%     \caption{Integrity of the model execution.}
%     \label{fig:model_integrity}
% \end{figure}



% \subsection{Model Protection}

% \myparagraph{Model Parameters}
% Protecting the model weights requires transmitting encrypted (and authenticated) parameters from the model provider to the NPU. However, the model cannot be executed with the encrypted parameters. Therefore, we include an additional layer before the hidden layer that first verifies the MAC of the parameters to ensure authenticity and then decrypts the model parameters using the AI CPU AES-GCM operator. Afterward, the model continues execution with the decrypted parameters.


% \begin{figure*}[!htpb]
%     \centering
%     \includegraphics[trim=0cm 13.7cm 12.5cm 0cm, clip,width=0.6\linewidth]{figures/npu_encrypted_model.pdf}
%     \caption{Encrypted model execution on NPU.}
%     \label{fig:npu_encrypted_model}
% \end{figure*}

% \myparagraph{Model Binary and Structure}
% Similar to the model parameters, the NPU runtime on the untrusted host model transfers the encrypted operator binaries to the NPU memory. The \texttt{PC\_START} attribute in the task points to the start address of the encrypted binary. Before the actual operator execution, the task scheduler schedules a custom AI CPU operator to decrypt the specific operator binary in place on the HBM.





% \begin{enumerate}
%     \item \textit{Host-side TEE} If there is a host-side TEE available, the model provider can simply encrypt the model file (which also contains the binary for the model operators) with the session secret (symmetric encryption key) between the TEE-VM and the model provider. This key can be generated after a successful remote attestation of the TEE-VM. 
%     \item \textit{No host-side TEE} If we assume there is no host side TEE available, or the host on the cloud provider is completely untrusted, the model provider can compile the AI CPU operator, generate the binary and extract the instructions from the binary that are corresponding to the operator. These compiled instructions can then be encrypted with the shard secret between the NPU and the model provider. After receiving the encrypted model binary, the NPU uses a trusted loader to load the encrypted binary, decrypt it and map it as executable memory. This way, the NPU can start executing the model. 
% \end{enumerate}


==> tables/compare.tex <==
\begin{tabular}{l|clccl|ll|ll|cl}
\hline
\multicolumn{1}{c|}{}                                                 & \multicolumn{5}{c|}{CC capability and trust assumption}                                                                                                                                                                                                                                                                                                                                                                & \multicolumn{2}{c|}{Device}                               & \multicolumn{2}{c|}{AI/ML Programming Capability}                                                                                                           & \multicolumn{2}{c}{Required changes}                                                                                                                                   \\ \cline{2-12} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Existing systems}}}      & Host TCB                                                                      & \multicolumn{1}{c}{{\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Isolation \\ granularity\end{tabular}}} & \begin{tabular}[c]{@{}c@{}}Spatial\\ Sharing\end{tabular} & \begin{tabular}[c]{@{}c@{}}Multi-residence\\ TEE\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Attestation*\\ (cpu/host excl.)\end{tabular}} & \multicolumn{1}{c}{Type} & \multicolumn{1}{c|}{Interface} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Native programming\\  interface\end{tabular}} & \multicolumn{1}{c|}{AI Stack}                                 & HW                                                                           & \multicolumn{1}{c}{SW}                                                                  \\ \hline
Graviton~\cite{volos2018graviton}                                     & Intel SGX + \notreq                                                           & \begin{tabular}[c]{@{}l@{}}GPU\\ contexts\end{tabular}                                                      & \supported                                                & \notsupported                                                 & HRoT,RA,STA                                                                                  & GPU                      & PCIe                           & CUDA                                                                                        & \begin{tabular}[c]{@{}l@{}}(CUDA \\ based)?\end{tabular}      & SC                                                                           & Runtime, Drivers,CUDA                                                                   \\
HIX~\cite{jang2019HIX}                                                & Intel SGX + \req                                                              & Enclaves                                                                                                    & \supported                                                & \notsupported                                                 & LA                                                                                           & GPU                      & PCIe                           & CUDA                                                                                        & ?                                                             & \begin{tabular}[c]{@{}c@{}}SGX instruction,\\ MMU, PCIe\end{tabular}         & \begin{tabular}[c]{@{}l@{}}GPU enclave, Inter-enclave\\ communication,CUDA\end{tabular} \\
GraphcoreIPU~\cite{vaswani2023confidential}                           & \notreq + Compiler                                                                     & Device                                                                                                      & \notsupported                                             & \supported                                                    & HRoT,SB,RA                                                                                   & IPU                      & PCIe                           & Proprietary                                                                                 & TF                                                            & CCU                                                                          & \begin{tabular}[c]{@{}l@{}}XLA, poplar compiler,\\ runtime\end{tabular}                 \\
NvidiaCC (H100)~\cite{h100}                                           & \begin{tabular}[c]{@{}c@{}}C-VM \\ + \req\end{tabular}                        & VM                                                                                                          & \supported                                                & \notsupported                                                 & HRoT,SB,RA                                                                                   & GPU                      & PCIe                           & CUDA                                                                                        & \begin{tabular}[c]{@{}l@{}}(CUDA\\ based)\end{tabular}        & \begin{tabular}[c]{@{}c@{}}Security\\ processor\end{tabular}                 & CUDA, C-VM?                                                                             \\
\cellcolor[HTML]{ECF4FF}{\color[HTML]{343434} Apple PCC~\cite{pcc} *} & ?                                                                             & Node                                                                                                        & ?                                                         & ?                                                             & HRoT,SB,RA                                                                                   & **                       & Internal*                      & (Swift)                                                                                     & \begin{tabular}[c]{@{}l@{}}Proprietary\\ support\end{tabular} & \begin{tabular}[c]{@{}c@{}}Custom Apple\\ Silicon\end{tabular}               & SepOS, SW stack                                                                         \\
sNPU~\cite{fen2024trusted}                                            & \begin{tabular}[c]{@{}c@{}}Penglai Enclave \\ +notreq + SM\end{tabular}       & Worlds                                                                                                      & \supported                                                & \notsupported                                                 & HRoT,SB                                                                                      & NPU                      & Internal                       & Proprietary                                                                                 & FS*                                                           & *                                                                            & *                                                                                       \\
StrongBox~\cite{deng2022strongbox}                                    & \begin{tabular}[c]{@{}c@{}}TrustZone\\ + \partreq + SM\end{tabular}           & Worlds                                                                                                      & \notsupported                                             & \notsupported                                                 & SB                                                                                           & GPU                      & Internal                       & OpenCL                                                                                      & FS*                                                           & -                                                                            & \begin{tabular}[c]{@{}l@{}}Runtime, Driver, \\ MMIO, TASK Protector\end{tabular}        \\
Honeycomb~\cite{mai2023honeycomb}                                     & \begin{tabular}[c]{@{}c@{}}AMD-SEV + \notreq \\ + Validator + SM\end{tabular} & \begin{tabular}[c]{@{}l@{}}SVSM \\ + SM\end{tabular}                                                        & \supported                                                & \notsupported                                                 & SB,RA(of SM)                                                                                 & GPU                      & PCIe                           & HIP                                                                                         & ?                                                             & -                                                                            & \begin{tabular}[c]{@{}l@{}}Validator, SVSM, \\ SM and runtime.\end{tabular}             \\
CAGE~\cite{wang2024cage}                                              & \begin{tabular}[c]{@{}c@{}}ARM CCA \\ + \partreq + SM\end{tabular}            & Realm                                                                                                       & \supported                                                & \notsupported                                                 & RA                                                                                           & GPU                      & PCIe                           & OpenCL                                                                                      & ?                                                             & -                                                                            & \begin{tabular}[c]{@{}l@{}}API, Monitors,\\ ShadowTask\end{tabular}                     \\
ACAI~\cite{sridhara2023acai}                                          & \begin{tabular}[c]{@{}c@{}}ARM CCA \\ + \req + PCIe port\end{tabular}         & Realm                                                                                                       & \notsupported                                             & \notsupported                                                 & SB,RA                                                                                        & GPU                      & PCIe                           & CUDA                                                                                        & ?                                                             & -                                                                            & \begin{tabular}[c]{@{}l@{}}TF-A, SMMU,\\  RMM\end{tabular}                              \\
GR-T~\cite{park2023safe}                                              & \begin{tabular}[c]{@{}c@{}}Trustzone \\ + \req + cloudVM\end{tabular}         & \begin{tabular}[c]{@{}l@{}}VM \\ + Worlds\end{tabular}                                                      & \supported                                                & \notsupported                                                 & SB,RA                                                                                        & GPU                      & Internal                       & GlobalPlatform API                                                                          & FS                                                            & -                                                                            & \begin{tabular}[c]{@{}l@{}}Driver Shim, \\ GPU\_shim\end{tabular}                        \\
HETEE~\cite{zhu2020hetee}                                             & \req* + SM                                                                    & Node                                                                                                        & \notsupported                                             & \notsupported                                                 & SB,RA                                                                                        & GPU                      & PCIe                           & Proprietary                                                                                 & FS                                                            & \begin{tabular}[c]{@{}c@{}}HETEE box, PCIe\\ interconnect, (SC)\end{tabular} & SC, API                                                                                 \\
ShEF~\cite{zhao2021shef}                                              & \notreq                                                                       & Device                                                                                                      & \notsupported                                             & \notsupported                                                 & SB,RA                                                                                        & FPGA                     & PCIe                           & Proprietary                                                                                 & ?                                                             & -                                                                            & ShEF Runtime, Shield                                                                    \\
\rowcolor[HTML]{FFCE93} 
\ascendcc                                                             & \notreq                                                                       & Device                                                                                                      & \cellcolor[HTML]{FFCE93}\notsupported                     & \supported                                                    & HRoT,SB,RA,TA                                                                                & NPU                      & PCIe                           & CANN                                                                                        & PT/TF                                                         & -                                                                            & \begin{tabular}[c]{@{}l@{}}Driver, Runtime, \\ Kernels (Operators)\end{tabular}        
\end{tabular}

==> tables/llama_results.tex <==
\begin{tabular}{@{}lllllllllllllllllllllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{Models}} & \multicolumn{24}{c}{Context Size}                                                                                                                                                                                                          \\ \cmidrule(l){2-25} 
\multicolumn{1}{c}{}                        & \multicolumn{3}{c}{128}     & \multicolumn{3}{c}{256}     & \multicolumn{3}{c}{512}     & \multicolumn{3}{c}{1024}    & \multicolumn{3}{c}{2048}    & \multicolumn{3}{c}{3072}    & \multicolumn{3}{c}{4096}    & \multicolumn{3}{c}{6114} \\ \cmidrule(l){2-25} 
\multicolumn{1}{c}{}                        & Vanilla & CC      & OH      & Vanilla & CC      & OH      & Vanilla & CC      & OH      & Vanilla & CC      & OH      & Vanilla & CC      & OH      & Vanilla & CC      & OH      & Vanilla & CC      & OH      & Vanilla    & CC   & OH   \\ \midrule
Llama-2-7b                                  & 5.17378 & 5.17399 & 0.00403 & 5.18651 & 5.18673 & 0.00425 & 5.99087 & 5.99827 & 0.00337 & 6.33594 & 6.33617 & 0.00360 & 6.87921 & 6.87945 & 0.00347 & 7.42954 & 7.42977 & 0.00303 & 8.33379 & 8.33400 & 0.00256 &            &      &      \\
Llama-2-7b-Chat-HF                          &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &            &      &      \\
Llama-2-13-Chat-HF                          &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &            &      &      \\
Llama-3-8b                                  &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &            &      &      \\
Llama-3-8b-Instruct                         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &            &      &      \\
Llama3-ChatQA-1.5-8B                        &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &         &            &      &      \\ \bottomrule
\end{tabular}
